Facts of US Firm Scale and Growth 1970-2019: An Illustrated Guide

This work analyzes data on all public US firms in the 50 year period 1970-2019, and presents 18 stylized facts of their scale, income, growth, return, investment, and dynamism. Special attention is given to (i) identifying distributional forms; and (ii) scale effects -- systematic difference between firms based on their scale of operations. Notable findings are that the Difference-of-Log-Normals (DLN) distribution has a central role in describing firm data, scale-dependent heteroskedasticity is rampant, and small firms are systematically different from large firms.

==> FigTab.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figures
\clearpage

% FSD stylized facts
\RPprep{Scale - Stylized facts}{0}{0}{FSDfacts}{%
    This figure presents stylized facts of the firm scale distribution (FSD). Panel (a) presents the number of firms per year. Panels (b) and (c) show the time trend of the FSD using real and GDP-adjusted dollars, respectively. For each year, the panels graph the $\{25,50,75\}^{th}$ percentiles of the FSD. Panels (d)-(f) present: un-adjusted equity scale FSD(EQ) w/ fitted Normal; time-adjusted equity scale FSD($\widetilde{\text{EQ}}$) w/ fitted Normal; and FSD($\widetilde{\text{EQ}}$) w/ fitted skew-Normal, respectively. Panels (g)-(i) present the respective q-q plots of panels (d)-(f).
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[Number of firms]{\includegraphics[width=2in]{Img/Num_Firms_Good.pdf}} & \subfigure[Time trend of FSD (real)]{\includegraphics[width=2in]{Img/FSD_Year_Index1_Good.pdf}} &
		\subfigure[Time trend of FSD (GDP)]{\includegraphics[width=2in]{Img/FSD_Year_Index2_Good.pdf}} \\ \\
		\subfigure[FSD(EQ) w/ N]{\includegraphics[width=2in]{Img/FSD_EQ_N_Good.pdf}} &
		\subfigure[FSD($\widetilde{\text{EQ}}$) w/ N]{\includegraphics[width=2in]{Img/FSD_EQt_N_Good.pdf}} &
		\subfigure[FSD($\widetilde{\text{EQ}}$) w/ SN]{\includegraphics[width=2in]{Img/FSD_EQt_SN_Good.pdf}} \\ \\
		\subfigure[q-q FSD(EQ) vs. N]{\includegraphics[width=2in]{Img/FSD_EQ_N_Good_qq.pdf}} &
		\subfigure[q-q FSD($\widetilde{\text{EQ}}$) vs. N]{\includegraphics[width=2in]{Img/FSD_EQt_N_Good_qq.pdf}} &
		\subfigure[q-q FSD($\widetilde{\text{EQ}}$) vs. SN]{\includegraphics[width=2in]{Img/FSD_EQt_SN_Good_qq.pdf}} \\ \\
	\end{tabular}
}



% FID stylized facts
\RPprep{Income - Stylized facts}{0}{0}{FIDfacts}{%
    This figure presents stylized facts of the firm income distribution (FID). Panel (a) presents the truncated distribution of FID(CF) in linear scale and Panel (b) presents the untruncated distribution in asinh scale, both overlaid with ML-fitted DLN distributions. Panel (c) presents the q-q for the fit of FID(CF) to the DLN distribution. Panels (d)-(f) repeat for owner income, FID(DI). Panel (g) presents the dependence of the FID on firm scale, by presenting the (10,25,50,75,90)$^{th}$ percentiles of FID(CF) conditional on the sign of CF, for 49 KT scale bins. Panel (h) presents the time- and scale-adjusted FID($\widetilde{\text{CF}}$), with scale adjustment done by considering intensity relative to total capital KT. Panel (i) presents the dependence of FID($\widetilde{\text{CF}}$) on firm scale. Panels (g)-(i) use the \{Non-Bank\} subset.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[FID(CF) w/ DLN ]{\includegraphics[width=2in]{Img/FID_CF_DLN_trunc_Good.pdf}} & \subfigure[FID(CF) w/ DLN ]{\includegraphics[width=2in]{Img/FID_CF_DLN_Good.pdf}} &
		\subfigure[q-q FID(CF) vs. DLN ]{\includegraphics[width=2in]{Img/FID_CF_DLN_Good_qq.pdf}} \\ \\
		\subfigure[FID(DI) w/ DLN ]{\includegraphics[width=2in]{Img/FID_DI_DLN_trunc_Good.pdf}} &
		\subfigure[FID(DI) w/ DLN ]{\includegraphics[width=2in]{Img/FID_DI_DLN_Good.pdf}} &
		\subfigure[q-q FID(DI) vs. DLN ]{\includegraphics[width=2in]{Img/FID_DI_DLN_Good_qq.pdf}} \\ \\
		\subfigure[FID(CF) by scale ]{\includegraphics[width=2in]{Img/FID_SCL_CF_Bank.pdf}} &
		\subfigure[FID($\widetilde{\text{CF}}$) w/ DLN ]{\includegraphics[width=2in]{Img/FID_CFt_DLN_Bank.pdf}} &
		\subfigure[FID($\widetilde{\text{CF}}$) by scale ]{\includegraphics[width=2in]{Img/FID_SCL_CF_adj_Bank.pdf}} \\ \\
	\end{tabular}
}



% FGD stylized facts
\RPprep{Growth - Stylized facts}{0}{0}{FGDfacts}{%
    This figure presents stylized facts of the firm growth distribution (FGD). Panel (a) presents the FGD(SL), with MLE- and LAD-fitted Normal distributions, and panels (b) and (c) present the respective q-q plots. Panel (d) presents the q-q plot of FGD(SL) vs. the DLN. Panel (e) presents the FGD time trend by plotting the $\{25,50,75\}^{th}$ percentiles of the FGD per year. Panel (f) plots binscatters of the median and IQR of FGD(SL) per 49 scale bins, ignoring the top and bottom 1\% of the data. Panel (g) presents the (10,25,50,75,90)$^{th}$ percentiles of FGD(SL) for the 49 scale bins. Panel (h) presents the time- and scale-adjusted FGD($\widetilde{\text{SL}}$), overlaid with an MLE-fitted DLN, and Panel (i) presents the respective q-q plot.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[FGD(SL) w/ Normals ]{\includegraphics[width=2in]{Img/FGD_SL_N_NL_Good.pdf}} & \subfigure[q-q FGD(SL) vs. Normal ]{\includegraphics[width=2in]{Img/FGD_SL_N_Good_qq.pdf}} &
		\subfigure[q-q FGD(SL) vs. Normal ]{\includegraphics[width=2in]{Img/FGD_SL_NL_Good_qq.pdf}} \\ \\
		\subfigure[q-q FGD(SL) vs. DLN ]{\includegraphics[width=2in]{Img/FGD_SL_DLN_Good_qq.pdf}} &
		\subfigure[Time trend of FGD ]{\includegraphics[width=2in]{Img/FGD_Year_SL_Index2_Good.pdf}} &
		\subfigure[FGD(SL) Median+IQR ]{\includegraphics[width=2in]{Img/FGD_MEDIQR_SL_Good.pdf}} \\ \\
		\subfigure[FGD(SL) by scale ]{\includegraphics[width=2in]{Img/FGD_SCL_SL_Good.pdf}} &
		\subfigure[FGD($\widetilde{\text{SL}}$) w/ DLN ]{\includegraphics[width=2in]{Img/FGD_SLt_DLN_Good.pdf}} &
		\subfigure[q-q FGD($\widetilde{\text{SL}}$) vs. DLN ]{\includegraphics[width=2in]{Img/FGD_SLt_DLN_Good_qq.pdf}} \\ \\
	\end{tabular}
}



% FGD - Decreasing dispersion
\RPprep{Growth - Decreasing dispersion}{0}{0}{FGDDisp}{%
    This figure presents the dependence of firm growth dispersion on firm scale. For each of the six firm size measures $XX=\{EQ,VL,KP,KT,SL,XS\}$, the sample is first split into $49$ equal bins, based on firm scale, $\log(XX)$, truncating the top and bottom 1\% of the FSD, such that each bin contains 2\% of the observations. For each bin, the corresponding panel presents the log of each bin's growth dispersion $\log(\text{IQR}[dlog(XX)])$ as a function of scale $\log(XX)$, along with fitted regression lines.
}
\RPfig{%
	\begin{tabular}{ccc}
		\subfigure[FGD(EQ)] {\includegraphics[width=2in]{Img/FGD_LIQR_EQ_Good.pdf}}
		& \subfigure[FGD(VL)]
		{\includegraphics[width=2in]{Img/FGD_LIQR_VL_Good.pdf}}
		& \subfigure[FGD(KP)]
		{\includegraphics[width=2in]{Img/FGD_LIQR_KP_Good.pdf}} \\ \\
		\subfigure[FGD(KT)] {\includegraphics[width=2in]{Img/FGD_LIQR_KT_Good.pdf}}
		& \subfigure[FGD(SL)]
		{\includegraphics[width=2in]{Img/FGD_LIQR_SL_Good.pdf}}
		& \subfigure[FGD(XS)]
		{\includegraphics[width=2in]{Img/FGD_LIQR_XS_Good.pdf}} \\ \\
	\end{tabular}
}



% FGD(EQ) stylized facts
\RPprep{Equity return - Stylized facts}{0}{0}{FGDEQfacts}{%
    This figure presents stylized facts of the equity return distribution FGD(EQ). Panel (a) presents median and IQR binscatters for yearly raw unadjusted returns per 49 scale bins, ignoring the top and bottom 1\% of the data, with scale defined as lagged log(EQ).Panels (b) and (c) present binscatters for monthly and daily excess unadjusted returns relative to FF3. Panels (d)-(f) present the histograms for the respective flavors, overlaid with fitted DLN distributions, and Panels (g)-(i) present the respective q-q plots vs. the DLN.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[Raw (Y) Median+IQR ]{\includegraphics[width=2in]{Img/FGDEQ_MEDIQR_year_lret_Good.pdf}} & \subfigure[FF3 (M) Median+IQR ]{\includegraphics[width=2in]{Img/FGDEQ_MEDIQR_month_lXret_Good.pdf}} &
		\subfigure[FF3 (D) Median+IQR ]{\includegraphics[width=2in]{Img/FGDEQ_MEDIQR_day_lXret_Good.pdf}} \\ \\
		\subfigure[Raw (Y) w/ DLN ]{\includegraphics[width=2in]{Img/FGDEQ_Y_ret_DLN.pdf}} &
		\subfigure[FF3 (M) w/ DLN ]{\includegraphics[width=2in]{Img/FGDEQ_M_Xret_DLN.pdf}} &
		\subfigure[FF3 (D) w/ DLN ]{\includegraphics[width=2in]{Img/FGDEQ_D_Xret_DLN.pdf}} \\ \\
		\subfigure[q-q Raw (Y) vs. DLN ]{\includegraphics[width=2in]{Img/FGDEQ_Y_ret_DLN_qq.pdf}} &
		\subfigure[q-q FF3 (M) vs. DLN ]{\includegraphics[width=2in]{Img/FGDEQ_M_Xret_DLN_qq.pdf}} &
		\subfigure[q-q FF3 (D) vs. DLN ]{\includegraphics[width=2in]{Img/FGDEQ_D_Xret_DLN_qq.pdf}} \\ \\
	\end{tabular}
}



% FIGD stylized facts
\RPprep{Income growth - Stylized facts}{0}{0}{FIGDfacts}{%
    This figure presents stylized facts of the firm income growth distribution (FIGD). Panel (a) presents the FIGD time trend by plotting the $\{25,50,75\}^{th}$ percentiles of FIGD(CF) per year. Panel (b) presents the FIGD(CF) histogram overlaid with an MLE-fitted DLN, and panel (c) presents the respective q-q plot. Panel (d) presents the (25,50,75)$^{th}$ percentiles of FIGD(CF) for the 49 scale bins, and panel (e) plots the binscatter of their dispersion. Panel (f) plots the percentiles of FIGD(DI), and panel (g) plots its histogram, fitted with a DLN. Panels (h) and (i) again present the FIGD(DI) histogram, but split the sample to growth from positive values and growth from negative values, respectively.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[Time trend of FIGD ]{\includegraphics[width=2in]{Img/FIGD_Year_CF_Index2_Good.pdf}} & \subfigure[FIGD(CF) w/ DLN ]{\includegraphics[width=2in]{Img/FIGD_CF_DLN_Good.pdf}} &
		\subfigure[q-q FIGD(CF) vs. DLN ]{\includegraphics[width=2in]{Img/FIGD_CF_DLN_Good_qq.pdf}} \\ \\
		\subfigure[FIGD(CF) by scale ]{\includegraphics[width=2in]{Img/FIGD_SCL_CF_Good.pdf}} &
		\subfigure[FIGD(CF) dispersion ]{\includegraphics[width=2in]{Img/FIGD_LIQR_CF_Good.pdf}} &
		\subfigure[FIGD(DI) by scale ]{\includegraphics[width=2in]{Img/FIGD_SCL_DI_Good.pdf}} \\ \\
		\subfigure[FIGD(DI) w/ DLN ]{\includegraphics[width=2in]{Img/FIGD_DI_DLN_Good.pdf}} &
		\subfigure[FIGD($\widetilde{\text{DI}})^{+}$ w/ DLN ]{\includegraphics[width=2in]{Img/FIGD_DIt_DLN_p_Good.pdf}} &
		\subfigure[FIGD($\widetilde{\text{DI}})^{-}$ w/ DLN ]{\includegraphics[width=2in]{Img/FIGD_DIt_DLN_n_Good.pdf}} \\ \\
	\end{tabular}
}



% FND stylized facts
\RPprep{Investment - Stylized facts}{0}{0}{FNDfacts}{%
    This figure presents stylized facts of the firm investment distribution (FND). Panels (a)+(d) present the total investment distribution FND(IT) overlaid with MLE-fitted DLN and its q-q plot. Panel (b)+(e) and (c)+(f) repeat for physical investment FND(IP) and for total investment intensity FND($\widetilde{\text{IT}})$, respectively. Panel (g) presents the dependence of the FND on firm scale, by presenting the (10,25,50,75,90)$^{th}$ percentiles of FND(IT) conditional on the sign of IT, for 49 KT scale bins. Panel (h) presents the dependence of investment intensity FND($\widetilde{\text{IT}})$ on scale. Panel (i) presents the dependence of physical depreciation intensity, DP/KP, on physical capital scale KP. All figures are based on the \{Non-Bank\} data subset.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[FND(IT) w/ DLN ]{\includegraphics[width=2in]{Img/FND_IT_DLN_Bank.pdf}} &     \subfigure[FND(IP) w/ DLN ]{\includegraphics[width=2in]{Img/FND_IP_DLN_Bank.pdf}} &
		\subfigure[FND($\widetilde{\text{IT}}$) w/ DLN ]{\includegraphics[width=2in]{Img/FND_ITt_DLN_Bank.pdf}} \\ \\
		\subfigure[q-q FND(IT) vs. DLN ]{\includegraphics[width=2in]{Img/FND_IT_DLN_Bank_qq.pdf}} &
		\subfigure[q-q FND(IP) vs. DLN ]{\includegraphics[width=2in]{Img/FND_IP_DLN_Bank_qq.pdf}} &
		\subfigure[q-q FND($\widetilde{\text{IT}}$) vs. DLN ]{\includegraphics[width=2in]{Img/FND_ITt_DLN_Bank_qq.pdf}} \\ \\
		\subfigure[FND(IT) by scale ]{\includegraphics[width=2in]{Img/FND_SCL_IT_Bank.pdf}} &
		\subfigure[FND($\widetilde{\text{IT}}$) by scale ]{\includegraphics[width=2in]{Img/FND_SCL_IT_adj_Bank.pdf}} &
		\subfigure[DP/KP by scale ]{\includegraphics[width=2in]{Img/FND_SCL_DP_Bank.pdf}} \\ \\
	\end{tabular}
}



% FRD stylized facts
\RPprep{R\&D - Stylized facts}{0}{0}{FRDfacts}{%
    This figure presents stylized facts of firm R\&D investment. Panel (a) presents the (log) R\&D investment distribution overlaid with MLE-fitted skew-Normal. Panels (b) and (c) repeat for (log) R\&D intensity relative to KT and SL, respectively. Panels (d) and (e) present the distribution of (log) R\&D intensity by KT scale, and its binned median and skewness. Panel (f) repeats panel (e) , but for (log) R\&D intensity relative to SL scale. Panels (g) and (h) present the distribution of (log) physical investment intensity IP by KT scale, and its binned median and skewness, but limits the sample to R\&D performing firms. Panel (i) repeats panel (h) for non-R\&D performing firms. All figures are based on the \{Non-Bank\} data subset.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[log(RD) w/ SN ]{\includegraphics[width=2in]{Img/FRD_RD_SN_Bank.pdf}} &     \subfigure[log(RD/KT) w/ SN ]{\includegraphics[width=2in]{Img/FRD_RD_KT_SN_Bank.pdf}} &
		\subfigure[log(RD/SL) w/ SN ]{\includegraphics[width=2in]{Img/FRD_RD_SL_SN_Bank.pdf}} \\ \\
		\subfigure[log(RD/KT) by scale ]{\includegraphics[width=2in]{Img/FRD_SCL_RD_KT_Bank.pdf}} &
		\subfigure[log(RD/KT) Med+Skew ]{\includegraphics[width=2in]{Img/FRD_MEDSK_RD_KT_Bank.pdf}} &
		\subfigure[log(RD/SL) Med+Skew ]{\includegraphics[width=2in]{Img/FRD_MEDSK_RD_SL_Bank.pdf}} \\ \\
		\subfigure[log(IP/KT) by scale ]{\includegraphics[width=2in]{Img/FRD_SCL_IP_RD_KT_Bank.pdf}} &
		\subfigure[log(IP/KT) Med+Skew ]{\includegraphics[width=2in]{Img/FRD_MEDSK_IP_RD_KT_Bank.pdf}} &
		\subfigure[log(IP/KT) Med+Skew ]{\includegraphics[width=2in]{Img/FRD_MEDSK_IP_NRD_KT_Bank.pdf}} \\ \\
	\end{tabular}
}



% DYN stylized facts
\RPprep{Dynamism - Stylized facts}{0}{0}{DYNfacts}{%
    This figure presents stylized facts of firm dynamism. Panel (a) graphs the $\{1,10,25,50,75,90,99\}^{th}$ percentiles of the 10-year ahead KT scale distribution per current scale bin. Panel (b) graphs percentiles of the age distribution by scale, and panel (c) percentiles of the scale distribution by age, along with a fitted median regression line. Panels (d) and (e) plot exit and entry probability by scale bin, respectively, and include exponential-fit trend lines. Panel (f) plots exit probability by age, along with a linear trend line. Panel (g) plots the (log) number of observations by age in the entire sample, along with the fitted trend line. Panel (g) presents the distribution of scale at entry and at exit, and panel (h) plots the probability of entry and exit by year, with the horizontal line the unconditional exit probability. All figures are based on the \{Non-Bank\} data subset.
}
\RPfig{%
	\begin{tabular}{ccc} 
		\subfigure[10-year forward scale ]{\includegraphics[width=2in]{Img/DYN_FSCL_SCL_KT_Bank.pdf}} &     \subfigure[Age dist. by scale ]{\includegraphics[width=2in]{Img/DYN_AGE_SCL_KT_Bank.pdf}} &
		\subfigure[Scale dist. by age ]{\includegraphics[width=2in]{Img/DYN_SCL_AGE_KT_Bank.pdf}} \\ \\
		\subfigure[Exit prob. by scale ]{\includegraphics[width=2in]{Img/DYN_XPROB_SCL_KT_Bank.pdf}} &
		\subfigure[Entry prob. by scale ]{\includegraphics[width=2in]{Img/DYN_NPROB_SCL_KT_Bank.pdf}} &
		\subfigure[Exit prob. by age ]{\includegraphics[width=2in]{Img/DYN_XPROB_AGE_Bank.pdf}} \\ \\
		\subfigure[log(\#obs) by age ]{\includegraphics[width=2in]{Img/DYN_XPROB_Uncond_Bank.pdf}} &
		\subfigure[Scale at entry/exit ]{\includegraphics[width=2in]{Img/DYN_SCL_ENTEXT_Bank.pdf}} &
		\subfigure[Entry/exit by year ]{\includegraphics[width=2in]{Img/DYN_XNPROB_YEAR_Bank.pdf}} \\ \\
	\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
\clearpage

\RPprep{Data definitions}{0}{0}{DataDef}{%
    This table defines all data items used. The first column is the name of each data item and the second is the mnemonic used throughout. The third column is the mapping to Compustat items or previously defined mnemonics, and the fourth is a short description. The core accounting identity used is the sources and uses equation: income = sales - expenses = total dividends + total investment, with dividends broadly defined below. The last two data items are alternative definitions, used for comparability with previous work. The ``L.'' is the lag operator.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{lllF}
    \toprule
    Name & XX & Definition & Description \\
    \midrule
    Equity value & EQ & mve & market, year end \\
    Debt value & DB & lt  & book total liabilities \\
    Total value & VL & EQ + DB & equity + debt \\
    Equity dividends & DE & dvt + (prstkc - sstk)  & dividends + net repurchase \\
    Debt dividends & DD & xint + (L.DB-DB) & interest paid + decrease in debt \\
    Total dividends & DI & DE + DD & to equity and debt \\
    Physical capital & KP & ppent & PP\&E, net of depreciation \\
    Total capital & KT & at & total assets (tangible) \\
    Depreciation & DP & dp & of physical capital \\
    Physical investment & IP & KP - L.KP + DP &  growth in net physical capital \\
    Total investment & IT & KT - L.KT + DP & growth in net assets \\
    Income & CF & DI + IT & bottom-up free cash flows \\
    Sales & SL & sl & total sales \\
    Expenses & XS & SL - CF & dissipated sales \\
    R\&D & RD & xrd & an expense included in XS \\
    Expenses (alt.) & XA & cogs + xsga + txt & top-down definition \\
    Income (alt.) & CA & SL - XA & top-down definition \\
    Investment (alt.) & IA & capx - sppe & cash-flow statement definition \\
	\bottomrule
    \end{tabularx}
}



\RPprep{Scale - Descriptive statistics}{0}{0}{FSDDescMom}{%
    Panel (a) of this table presents the first four central moments of the FSD, based on six measures of size. Variable definitions are in Table~\ref{tab:DataDef}. Time-adjusted versions are marked with $\widetilde{XX}$, and time-adjustment procedure is described in Appendix~\ref{sec:AppdxFE}. The panel also presents the persistence of each measure, using the \cite{ArellanoBover1995}/\cite{BlundellBond1998} panel estimator. Panel (b) presents the correlations between the measures, with the upper triangular presenting correlations between unadjusted measures (XX) and the lower triangular correlations between time-adjusted measures ($\widetilde{\text{XX}}$). Panel (c) presents the results of three cointegration tests between all FSD panels, with the first two tests from \cite{Pedroni2004}, and the third from \cite{Westerlund2005}. The first two test the null of no cointegration vs. the alternative that all panels are cointegrated while the third tests vs. the alternative that some panels are cointegrated. Tests are conducted by decade, on the available balanced sample of time-adjusted measures within each decade.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	\multicolumn{13}{l}{\textit{Panel (a): Scale = log(XX) moments}}\\
	\midrule
	& EQ & VL & KP & KT & SL & XS & $\widetilde{\text{EQ}}$ & $\widetilde{\text{VL}}$ & $\widetilde{\text{KP}}$ & $\widetilde{\text{KT}}$ & $\widetilde{\text{SL}}$ & $\widetilde{\text{XS}}$\\
	\midrule
    $M_{1}$ (mean) & 6.19 & 6.98 & 4.91 & 6.65 & 6.36 & 6.30 & 6.19 & 7.01 & 4.96 & 6.69 & 6.40 & 6.34 \\
    $M_{2}$ (s.d.) & 2.16 & 2.12 & 2.41 & 2.11 & 2.13 & 2.05 & 2.20 & 2.17 & 2.43 & 2.14 & 2.13 & 2.06 \\
    $M_{3}$ (skew) & 0.27 & 0.34 & 0.32 & 0.36 & 0.09 & 0.23 & 0.30 & 0.37 & 0.37 & 0.41 & 0.16 & 0.29 \\
    $M_{4}$ (kurt) & 2.75 & 2.91 & 2.56 & 2.99 & 2.86 & 2.78 & 2.81 & 2.96 & 2.66 & 3.02 & 2.92 & 2.87 \\ \\
    Persistence & 0.87 & 0.93 & 1.18 & 1.15	& 1.01 & 0.76 & 0.97 & 0.98 & 0.98 & 1.01 & 0.92 & 0.84 \\
    s.e.        & .003 & .002 & .003 & .002 & .004 & .004 & .003 & .002 & .002 & .001 & .002 & .003 \\
    \end{tabularx}

    \begin{tabularx}{3.2in}{Frrrrrr}
	\\ \multicolumn{7}{l}{\textit{Panel (b): Scale correlations}}\\
	\midrule
	& EQ & VL & KP & KT & SL & XS \\
	\midrule
	EQ &  --- & .941 & .779 & .864 & .809 & .799 \\
	VL & .938 &  --- & .822 & .967 & .850 & .837 \\
	KP & .804 & .845 &  --- & .854 & .852 & .834 \\
	KT & .864 & .968 & .869 &  --- & .877 & .860 \\
	SL & .830 & .867 & .848 & .885 &  --- & .982 \\
	XS & .819 & .853 & .829 & .867 & .982 &  --- \\
    \end{tabularx}

    \begin{tabularx}{\linewidth}{Fcccccc}
	\\ \multicolumn{7}{l}{\textit{Panel (c): Scale cointegration tests}}\\
	\midrule
	& Phillips-Perron t & p-val & Dicky-Fuller t & p-val & Variance ratio & p-val \\
	70's & 51.12 & $<$0.001 & -65.76 & $<$0.001 & 17.42 & $<$0.001 \\
	80's & 57.38 & $<$0.001 & -57.41 & $<$0.001 & 21.32 & $<$0.001 \\
	90's & 58.97 & $<$0.001 & -65.87 & $<$0.001 & 22.05 & $<$0.001 \\
	00's & 62.51 & $<$0.001 & -75.13 & $<$0.001 & 21.67 & $<$0.001 \\
	10's & 58.97 & $<$0.001 & -60.87 & $<$0.001 & 22.57 & $<$0.001 \\
    \bottomrule
    \end{tabularx}
}



\RPprep{Scale - Distributional tests}{1}{0}{FSDdist}{%
    This table presents results of tests of distribution equality for the FSD, based on the scale measures described in Table~\ref{tab:DataDef}. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a) and (b) report the test statistics and their p-values for the Normal and skew-Normal, respectively. Panel (c) reports the AIC- and BIC-based relative likelihoods for each distribution.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	& EQ & VL & KP$^{a}$ & KT$^{a}$ & SL & XS & $\widetilde{\text{EQ}}$ & $\widetilde{\text{VL}}$ & $\widetilde{\text{KP}}^{a}$ & $\widetilde{\text{KT}}^{a}$ & $\widetilde{\text{SL}}$ & $\widetilde{\text{XS}}$\\ 
	\midrule
	\\ \multicolumn{13}{l}{\textit{Panel (a): FSD vs. Normal}}\\
	\midrule
    K-S   & 0.029 & 0.026 & 0.023 & 0.028 & 0.010 & 0.022 & 0.029 & 0.031 & 0.028 & 0.034 & 0.017 & 0.028 \\
    p-val & 0.025 & 0.029 & 0.032 & 0.026 & 0.059 & 0.033 & 0.026 & 0.024 & 0.027 & 0.022 & 0.041 & 0.027 \\
    C-2   & 191   & 200   & 207   & 230   & 47    & 160   & 202   & 233   & 261   & 329   & 88    & 221   \\
    p-val & 0.027 & 0.027 & 0.026 & 0.025 & 0.054 & 0.030 & 0.027 & 0.025 & 0.023 & 0.020 & 0.040 & 0.025 \\ 
    A-D   & 17.18 & 16.91 & 16.15 & 19.70 & 2.89  & 11.92 & 18.40 & 21.62 & 20.84 & 28.26 & 7.08  & 18.47 \\
    p-val & 0.026 & 0.027 & 0.027 & 0.025 & 0.052 & 0.031 & 0.026 & 0.024 & 0.024 & 0.021 & 0.038 & 0.026 \\ 
    \\ \multicolumn{13}{l}{\textit{Panel (b): FSD vs. skew-Normal}}\\
	\midrule
    K-S   & 0.011 & 0.009 & 0.015 & 0.008 & 0.006 & 0.010 & 0.006 & 0.005 & 0.014 & 0.007 & 0.005 & 0.007 \\
    p-val & 0.056 & 0.066 & 0.045 & 0.069 & 0.086 & 0.058 & 0.086 & 0.098 & 0.048 & 0.074 & 0.099 & 0.075 \\
    C-2   & 22.47 & 30.51 & 99    & 32    & 22.26 & 41.73 & 16.82 & 17.65 & 67    & 30    & 17.73 & 23.27 \\
    p-val & 0.077 & 0.066 & 0.038 & 0.064 & 0.077 & 0.057 & 0.089 & 0.087 & 0.046 & 0.067 & 0.087 & 0.075 \\ 
    A-D   & 2.163 & 1.639 & 7.660 & 1.410 & 0.681 & 2.252 & 1.061 & 0.599 & 4.410 & 1.160 & 0.534 & 1.106 \\
    p-val & 0.057 & 0.062 & 0.037 & 0.065 & 0.081 & 0.056 & 0.070 & 0.084 & 0.045 & 0.069 & 0.087 & 0.070 \\ 
    \\ \multicolumn{13}{l}{\textit{Panel (c): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Normal  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Skew-N & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Normal  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Skew-N & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
    \begin{flushleft}
    $^a$ Using the \{Non-Bank\} data subset \\
    \end{flushleft}    
}



\RPprep{Income - Descriptive statistics}{0}{0}{FIDDescMom}{%
    The first four columns of this table present statistics for the positive side of the FID, while the next four concentrate on the negative side and the last four on the entire income intensity distribution (i.e., income divided by total capital KT). Variable definitions are in Table~\ref{tab:DataDef}. The positive and negative sides are in asinh scale. $M_1$ to $M_4$ are the first four central moments. Persistence for the positives and negatives is the 1-lag pooled auto-correlation, while for intensities it is the \cite{ArellanoBover1995}/\cite{BlundellBond1998} panel estimate. \%Ob is the percent of total observations in the positive/negative side, and may not sum to 100\% due to zero-valued obs. The scaling coefficient is the slope in a quantile regression of (asinh) income or of intensity on scale.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	& CF$^{+}$ & CA$^{+}$ & DI$^{+}$ & DE$^{+}$ & CF$^{-}$ & CA$^{-}$ & DI$^{-}$ & DE$^{-}$ & $\widetilde{\text{CF}}$ & $\widetilde{\text{CA}}$ & $\widetilde{\text{DI}}$ & $\widetilde{\text{DE}}$\\
	\midrule
    $M_{1}$ & 5.02 & 5.00 & 4.88 & 3.94 & -3.59 & -3.04 & -4.53 & -2.57 & 0.07  & 0.09  & -0.02 & -0.02  \\
    $M_{2}$ & 2.15 & 2.06 & 2.24 & 2.30 & 1.90  & 1.58  & 2.19  & 2.09  & 0.20  & 0.18  & 0.33  & 0.22   \\
    $M_{3}$ & 0.20 & 0.26 & 0.20 & 0.30 & -0.52 & -0.37 & -0.34 & -0.61 & -0.06 & -3.19 & -4.72 & -9.20  \\
    $M_{4}$ & 2.73 & 2.88 & 2.76 & 2.44 & 3.37  & 3.20  & 3.15  & 2.50  & 47    & 69    & 46    & 135    \\
    Pers.   & 0.59 & 0.80 & 0.33 & 0.62 & -0.10 & 0.20  & 0.01  & -0.02 & 0.16  & 0.48  & 0.04  & 0.06   \\
    \%Ob  & 0.80 & 0.75 & 0.59 & 0.56 & 0.20  & 0.11  & 0.41  & 0.33  & /     & /     & /     & /      \\
    $\beta_{scl}$ & 0.96 & 0.99 & 0.97 & 0.98 & -0.70 & -0.68 & -0.87 & -0.73 & 0.00  & 0.00  & 0.00  & 0.00   \\
    \end{tabularx}
}



\RPprep{Income - Distributional tests}{1}{0}{FIDdist}{%
    This table presents results of tests of distribution equality for the four measures of income: CF, CA, DI, and DE, described in Table~\ref{tab:DataDef}, as well as their time- and scale-adjusted versions. Scale adjustments use total capital (KT) as the size measure. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a)-(c) report the test statistics and their p-values for the Stable, Laplace, and DLN, respectively. Panel (d) reports the relative likelihoods for each distribution. The raw variables (columns 1-4) use the \{Good\} data subset. The scale adjusted versions use the \{Non-Bank\} subset.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrr}
    \toprule
	& CF & CA & DI & DE & $\widetilde{\text{CF}}$ & $\widetilde{\text{CA}}$ & $\widetilde{\text{DI}}$ & $\widetilde{\text{DE}}$\\ 
	\midrule
	\\ \multicolumn{9}{l}{\textit{Panel (a): Income vs. Stable}}\\
	\midrule
    K-S   & 0.035 & 0.033 & 0.023 & 0.041 & 0.040 & 0.050 & 0.055 & 0.096 \\
    p-val & 0.021 & 0.022 & 0.032 & 0.017 & 0.018 & 0.013 & 0.011 & 0.001 \\
    C-2   & 698   & $>$999& 364   & $>$999& 366   & 677   & 523   & $>$999\\
    p-val & 0.011 & 0.007 & 0.019 & 0.005 & 0.019 & 0.011 & 0.014 & 0.003 \\ 
    A-D   & 23.66 & 29.03 & 17.27 & 45.30 & 24.57 & 39.41 & 31.26 & 224.9 \\
    p-val & 0.023 & 0.020 & 0.026 & 0.016 & 0.022 & 0.017 & 0.020 & 0.001 \\ 
    \\ \multicolumn{9}{l}{\textit{Panel (b): Income vs. Laplace}}\\
	\midrule
    K-S   & 0.365 & 0.401 & 0.260 & 0.369 & 0.071 & 0.071 & 0.123 & 0.268 \\
    p-val & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.006 & 0.000 & 0.000 \\
    C-2   & $>$999& $>$999& $>$999& $>$999& 885   & 953   & $>$999& $>$999\\
    p-val & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 & 0.008 & 0.000 & 0.000 \\ 
    A-D   & $>$999& $>$999& $>$999& $>$999& 54.48 & 55.89 & 190.4 & 761.2 \\
    p-val & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 & 0.013 & 0.002 & 0.000 \\
    \\ \multicolumn{9}{l}{\textit{Panel (c): Income vs. DLN}}\\
	\midrule
    K-S   & 0.005 & 0.004 & 0.004 & 0.030 & 0.010 & 0.022 & 0.006 & 0.132 \\
    p-val & 0.092 & 0.108 & 0.120 & 0.024 & 0.061 & 0.033 & 0.088 & 0.000 \\
    C-2   & 16    & 16    & 11    & 183   & 57    & 152   & 20    & $>$999\\
    p-val & 0.092 & 0.091 & 0.117 & 0.028 & 0.049 & 0.031 & 0.082 & 0.000 \\ 
    A-D   & 0.70  & 0.39  & 0.29  & 10.36 & 1.86  & 7.36  & 0.47  & 204.08\\
    p-val & 0.080 & 0.095 & 0.105 & 0.033 & 0.059 & 0.037 & 0.090 & 0.001 \\
    \\ \multicolumn{9}{l}{\textit{Panel (d): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
}



\RPprep{Growth - Descriptive statistics}{0}{0}{FGDDescMom}{%
    Panel (a) of this table presents the first four central moments of the firm growth distribution (FGD), based on six measures of size. Variable definitions are in Table~\ref{tab:DataDef}. Time- and scale-adjusted versions are marked with $\widetilde{XX}$, and the adjustment procedure is described in Appendix~\ref{sec:AppdxFE}. The panel also presents the persistence of each growth measure, using the \cite{ArellanoBover1995}/\cite{BlundellBond1998} panel estimator. Panel (b) presents the correlations between the growth measures, with the upper triangular presenting correlations between unadjusted measures (XX) and the lower triangular correlations between time- and scale-adjusted measures ($\widetilde{\text{XX}}$).
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	\multicolumn{13}{l}{\textit{Panel (a): Growth = dlog(XX) moments}}\\
	\midrule
	& EQ & VL & KP & KT & SL & XS & $\widetilde{\text{EQ}}$ & $\widetilde{\text{VL}}$ & $\widetilde{\text{KP}}$ & $\widetilde{\text{KT}}$ & $\widetilde{\text{SL}}$ & $\widetilde{\text{XS}}$\\
	\midrule
    $M_{1}$ & -0.02 &  0.02 &  0.01 &  0.01 &  0.01 &  0.02 & -0.01 &  0.02 &  0.00 &  0.01 &  0.01 &  0.01 \\
    $M_{2}$ &  0.57 &  0.34 &  0.33 &  0.24 &  0.30 &  0.37 &  0.54 &  0.30 &  0.31 &  0.23 &  0.27 &  0.34 \\
    $M_{3}$ & -0.71 & -0.41 & -0.36 &  0.31 & -0.54 & -0.04 & -0.79 & -0.52 & -2.76 & -0.34 & -2.46 & -1.64 \\
    $M_{4}$ &  8.84 &  13.3 &  27.2 &  16.5 &  35.6 &  28.3 &  8.56 &  10.8 &  64.4 &  23.1 &  53.5 &  32.3 \\ \\
    Pers.   & -0.05 & -0.08 &  0.16 &  0.16 &  0.07 & -0.17 & -0.01 & -0.03 &  0.15 &  0.16 &  0.11 & -0.13 \\
    s.e.    & .002 & .002 & .003 & .003 & .003 & .002 & .002 & .002 & .003 & .003 & .003 & .002 \\
    \end{tabularx}

    \begin{tabularx}{3.2in}{Frrrrrr}
	\\ \multicolumn{7}{l}{\textit{Panel (b): Growth correlations}}\\
	\midrule
	& EQ & VL & KP & KT & SL & XS \\
	\midrule
	EQ &  --- & .867 & .136 & .324 & .203 & .001 \\
	VL & .871 &  --- & .113 & .316 & .191 & .004 \\
	KP & .138 & .104 &  --- & .579 & .376 & .214 \\
	KT & .306 & .275 & .611 &  --- & .501 & .198 \\
	SL & .234 & .207 & .416 & .530 &  --- & .514 \\
	XS & .022 & .026 & .217 & .209 & .584 &  --- \\
    \end{tabularx}
}



\RPprep{Growth - Distributional tests}{1}{0}{FGDdist}{%
    This table presents results of tests of distribution equality for the FGD, based on the scale measures described in Table~\ref{tab:DataDef}, as well as their time- and scale-adjusted versions, denoted $\widetilde{XX}$. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a)-(c) report the test statistics and their p-values for the Stable, Laplace, and DLN, respectively. Panel (d) reports the relative likelihoods for each distribution.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	& EQ & VL & KP$^{a}$ & KT$^{a}$ & SL & XS & $\widetilde{\text{EQ}}$ & $\widetilde{\text{VL}}$ & $\widetilde{\text{KP}}^{a}$ & $\widetilde{\text{KT}}^{a}$ & $\widetilde{\text{SL}}$ & $\widetilde{\text{XS}}$\\ 
	\midrule
	\\ \multicolumn{13}{l}{\textit{Panel (a): FGD vs. Stable}}\\
	\midrule
    K-S   & 0.013 & 0.017 & 0.016 & 0.011 & 0.012 & 0.009 & 0.012 & 0.019 & 0.021 & 0.012 & 0.013 & 0.011 \\
    p-val & 0.050 & 0.040 & 0.042 & 0.055 & 0.052 & 0.067 & 0.053 & 0.036 & 0.034 & 0.052 & 0.050 & 0.056 \\
    C-2   & 115   & 324   & 107   & 91    & 88    & 67    & 80    & 230   & 193   & 88    & 80    & 59    \\
    p-val & 0.036 & 0.020 & 0.037 & 0.040 & 0.040 & 0.046 & 0.042 & 0.025 & 0.027 & 0.041 & 0.042 & 0.049 \\ 
    A-D   & 4.37  & 10.60 & 6.73  & 3.79  & 4.04  & 2.77  & 3.34  & 9.36  & 14.93 & 3.70  & 4.31  & 3.50  \\
    p-val & 0.045 & 0.032 & 0.039 & 0.047 & 0.046 & 0.052 & 0.049 & 0.034 & 0.028 & 0.048 & 0.045 & 0.048 \\ 
    \\ \multicolumn{13}{l}{\textit{Panel (b): FGD vs. Laplace}}\\
	\midrule
    K-S   & 0.009 & 0.040 & 0.046 & 0.027 & 0.041 & 0.047 & 0.016 & 0.023 & 0.041 & 0.019 & 0.034 & 0.043 \\
    p-val & 0.063 & 0.018 & 0.015 & 0.027 & 0.017 & 0.014 & 0.043 & 0.032 & 0.017 & 0.036 & 0.022 & 0.016 \\
    C-2   & 52    & 368   & 509   & 290   & 415   & 657   & 98    & 121   & 320   & 137   & 225   & 436   \\
    p-val & 0.052 & 0.019 & 0.015 & 0.022 & 0.017 & 0.012 & 0.038 & 0.035 & 0.020 & 0.033 & 0.025 & 0.016 \\ 
    A-D   & 1.69  & 23.97 & 37.45 & 18.72 & 33.79 & 51.45 & 4.43  & 8.21  & 23.19 & 8.19  & 17.01 & 33.23 \\
    p-val & 0.061 & 0.023 & 0.018 & 0.025 & 0.019 & 0.014 & 0.045 & 0.036 & 0.023 & 0.036 & 0.027 & 0.019 \\ 
    \\ \multicolumn{13}{l}{\textit{Panel (c): FGD vs. DLN}}\\
	\midrule
    K-S   & 0.004 & 0.008 & 0.015 & 0.006 & 0.003 & 0.001 & 0.001 & 0.005 & 0.018 & 0.005 & 0.005 & 0.003 \\
    p-val & 0.129 & 0.069 & 0.045 & 0.087 & 0.155 & 0.748 & 0.819 & 0.106 & 0.039 & 0.096 & 0.096 & 0.165 \\
    C-2   & 9     & 39    & 105   & 17    & 7     & 5     & 5     & 14    & 167   & 12    & 11    & 5     \\
    p-val & 0.133 & 0.059 & 0.037 & 0.089 & 0.171 & 0.430 & 0.438 & 0.100 & 0.030 & 0.110 & 0.115 & 0.270 \\ 
    A-D   & 0.23  & 1.08  & 4.47  & 0.50  & 0.15  & 0.06  & 0.02  & 0.46  & 7.77  & 0.47  & 0.39  & 0.11  \\
    p-val & 0.112 & 0.070 & 0.045 & 0.089 & 0.130 & 0.184 & 0.349 & 0.091 & 0.037 & 0.090 & 0.095 & 0.144 \\ 
    \\ \multicolumn{13}{l}{\textit{Panel (d): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
    \begin{flushleft}
    $^a$ Using the \{Non-Bank\} data subset \\
    \end{flushleft}
}



\RPprep{Equity return - Descriptive statistics}{0}{1}{FGDEQDescMom}{%
    This table presents the first four central moments, as well as the median and IQR, of the firm equity return distribution FGD(EQ). Twelve flavors are presented: \{yearly,monthly,daily\}X\{raw,excess\}X\{unadjusted,adjusted\}. The returns are split and dividend adjusted, at the relevant horizon, with excess returns calculated relative the the Fama-French 3-factor model. The data are the CRSP universe 1970-2019. Time- and scale-adjusted versions are marked with $\widetilde{XXX}$, and the adjustment procedure is described in Appendix~\ref{sec:AppdxFE}.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	& \multicolumn{4}{c}{Yearly} & \multicolumn{4}{c}{Monthly} & \multicolumn{4}{c}{Daily} \\
	& Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ & Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ & Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ \\
	\midrule
    $M_{1}$ & -0.0072 & -0.1018 & 0.0131  & -0.0899 & -0.0004 & -0.0084 & 0.0008  & -0.0089 & -0.0001 & -0.0005 & 0.0004  & -0.0003  \\
    $M_{2}$ & 0.6227  & 0.6058  & 0.5763  & 0.5395  & 0.1658  & 0.1578  & 0.1513  & 0.1404  & 0.0471  & 0.0461  & 0.0387  & 0.0362   \\
    $M_{3}$ & -2.6784 & -2.5665 & -2.0654 & -1.9818 & -0.7209 & -0.5199 & -0.8319 & -0.9166 & -0.2377 & -0.2086 & -0.4708 & -0.5924  \\
    $M_{4}$ & 92      & 105     & 33      & 32      & 26      & 35      & 33      & 35      & 356     & 390     & 296     & 307      \\
    MED     & 0.0701  & -0.0341 & 0.0674  & -0.0363 & 0.0053  & -0.0035 & 0.0037  & -0.0048 & 0.0000  & -0.0005 & 0.0000  & -0.0005  \\
    IQR     & 0.5140  & 0.4695  & 0.4997  & 0.4627  & 0.1277  & 0.1140  & 0.1277  & 0.1155  & 0.0260  & 0.0237  & 0.0267  & 0.0245   \\
    \end{tabularx}
}



\RPprep{Equity return - Distributional tests}{1}{0}{FGDEQdist}{%
    This table presents results of tests of distribution equality for the following flavors of the FGD(EQ): \{yearly,monthly,daily\}X\{raw,excess\}X\{unadjusted,adjusted\}. Excess returns relative the the Fama-French 3-factor model are denoted FF3. Time- and scale-adjusted versions are marked with $\widetilde{XXX}$. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a)-(c) report the test statistics and their p-values for the Stable, Laplace, and DLN, respectively. Panel (d) reports the relative likelihoods for each distribution.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrrr}
    \toprule
	& \multicolumn{4}{c}{Yearly} & \multicolumn{4}{c}{Monthly} & \multicolumn{4}{c}{Daily} \\
	& Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ & Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ & Raw & FF3 & $\widetilde{\text{Raw}}$ & $\widetilde{\text{FF3}}$ \\
	\midrule
    \\ \multicolumn{13}{l}{\textit{Panel (a): FGD(EQ) vs. Stable}}\\
	\midrule
    K-S   & 0.017 & 0.017 & 0.015 & 0.015 & 0.013 & 0.015 & 0.011 & 0.013 & 0.021 & 0.014 & 0.014 & 0.015  \\
    p-val & 0.040 & 0.041 & 0.044 & 0.044 & 0.049 & 0.045 & 0.056 & 0.050 & 0.035 & 0.046 & 0.047 & 0.043  \\
    C-2   & 236   & 258   & 126   & 180   & 173   & 195   & 108   & 154   & 359   & 201   & 178   & 204    \\
    p-val & 0.024 & 0.023 & 0.034 & 0.028 & 0.029 & 0.027 & 0.037 & 0.031 & 0.019 & 0.027 & 0.029 & 0.027  \\
    A-D   & 8.54  & 9.12  & 4.88  & 6.74  & 6.07  & 6.67  & 4.18  & 5.75  & 8.32  & 6.16  & 5.77  & 6.70   \\
    p-val & 0.035 & 0.034 & 0.043 & 0.039 & 0.040 & 0.039 & 0.046 & 0.041 & 0.036 & 0.040 & 0.041 & 0.039  \\
    \\ \multicolumn{13}{l}{\textit{Panel (b): FGD(EQ) vs. Laplace}}\\
	\midrule
    K-S   & 0.027 & 0.030 & 0.016 & 0.015 & 0.023 & 0.026 & 0.013 & 0.013 & 0.045 & 0.051 & 0.025 & 0.027  \\
    p-val & 0.028 & 0.024 & 0.042 & 0.044 & 0.032 & 0.028 & 0.048 & 0.048 & 0.015 & 0.012 & 0.029 & 0.027  \\
    C-2   & 134   & 203   & 72    & 55    & 163   & 244   & 62    & 58    & 714   & 761   & 159   & 182    \\
    p-val & 0.033 & 0.027 & 0.044 & 0.050 & 0.030 & 0.024 & 0.048 & 0.049 & 0.011 & 0.010 & 0.030 & 0.028  \\
    A-D   & 9.21  & 14.66 & 4.00  & 3.92  & 12.62 & 19.38 & 4.52  & 5.27  & 50.80 & 62.69 & 15.26 & 17.40  \\
    p-val & 0.034 & 0.028 & 0.046 & 0.047 & 0.030 & 0.025 & 0.044 & 0.042 & 0.014 & 0.012 & 0.028 & 0.026  \\
    \\ \multicolumn{13}{l}{\textit{Panel (c): FGD(EQ) vs. DLN}}\\
	\midrule
    K-S   & 0.004 & 0.004 & 0.002 & 0.003 & 0.004 & 0.003 & 0.002 & 0.003 & 0.046 & 0.013 & 0.006 & 0.007  \\
    p-val & 0.113 & 0.115 & 0.256 & 0.166 & 0.115 & 0.148 & 0.277 & 0.148 & 0.015 & 0.050 & 0.084 & 0.080  \\
    C-2   & 10    & 12    & 3     & 6     & 8     & 5     & 2     & 9     & 729   & 60    & 18    & 21     \\
    p-val & 0.123 & 0.111 & 0.962 & 0.199 & 0.152 & 0.353 & 1.000 & 0.136 & 0.011 & 0.048 & 0.086 & 0.078  \\
    A-D   & 0.38  & 0.42  & 0.03  & 0.13  & 0.13  & 0.10  & 0.05  & 0.19  & 37.20 & 1.74  & 0.28  & 0.47   \\
    p-val & 0.096 & 0.093 & 0.297 & 0.138 & 0.137 & 0.148 & 0.199 & 0.120 & 0.018 & 0.061 & 0.105 & 0.090  \\
\\ \multicolumn{13}{l}{\textit{Panel (d): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
}



\RPprep{Income growth - Descriptive statistics}{0}{0}{FIGDDescMom}{%
    Panel (a) of this table presents the first four central moments and the median of the firm income growth distribution (FIGD), based on the four measures of income from Table~\ref{tab:FIDdist} and the DLN growth measure of \cite{Parham2022a}. Time- and scale-adjusted versions (relative to total capital KT) are marked with $\widetilde{XX}$, and the adjustment procedure is described in Appendix~\ref{sec:AppdxFE}. Panels (b) and (c) condition on the sign of beginning-of-period values, such that Panel (b) considers the distribution of income growth from initial positive income values and Panel (c) on income growth from initial negative income values.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrr}
    \toprule
	& CF & CA & DI & DE & $\widetilde{\text{CF}}$ & $\widetilde{\text{CA}}$ & $\widetilde{\text{DI}}$ & $\widetilde{\text{DE}}$\\ 
	\midrule
    \\ \multicolumn{9}{l}{\textit{Panel (a): All observations}}\\
	\midrule
    $M_{1}$ & 0.1910  & 0.0429  & 0.3102  & 0.1328  & 0.1956  & 0.0463  & 0.2857  & 0.1231   \\
    $M_{2}$ & 1.4549  & 0.6568  & 2.9249  & 1.9885  & 1.4661  & 0.6096  & 2.9196  & 2.1924   \\
    $M_{3}$ & 1.5010  & 0.0776  & 1.3826  & -0.3515 & 1.8638  & 0.4423  & 1.3225  & -0.4057  \\
    $M_{4}$ & 12.77   & 10.20   & 12.23   & 17.20   & 14.22   & 10.39   & 12.18   & 17.61    \\
    Med     & 0.0384  & 0.0351  & -0.0642 & 0.0219  & 0.0395  & 0.0348  & -0.0781 & 0.0199   \\
    \\ \multicolumn{9}{l}{\textit{Panel (b): Conditional on beginning positive}}\\
	\midrule
    $M_{1}$ & 0.0093  & -0.0051 & -0.2018 & -0.0130 & 0.0240  & 0.0067  & -0.2197 & -0.0292  \\
    $M_{2}$ & 1.0958  & 0.5207  & 2.4838  & 1.5073  & 1.1252  & 0.5038  & 2.4857  & 1.7336   \\
    $M_{3}$ & 0.7635  & -0.8674 & 1.4885  & 0.6271  & 1.0839  & -0.3578 & 1.4130  & 0.0673   \\
    $M_{4}$ & 12.06   & 9.94    & 14.16   & 16.56   & 12.45   & 8.83    & 14.03   & 17.14    \\
    Med     & -0.0073 & 0.0248  & -0.4012 & -0.0406 & -0.0064 & 0.0234  & -0.4158 & -0.0618  \\
    \\ \multicolumn{9}{l}{\textit{Panel (c): Conditional on beginning negative}}\\
	\midrule
    $M_{1}$ & 1.2514  & 0.5799  & 1.0553  & 0.4629  & 1.2126  & 0.5006  & 1.0204  & 0.4897   \\
    $M_{2}$ & 2.9827  & 1.7058  & 3.3746  & 3.2869  & 3.0355  & 1.5580  & 3.3585  & 3.4147   \\
    $M_{3}$ & 1.8312  & 0.3717  & 1.2318  & -1.5929 & 2.3865  & 1.1673  & 1.1591  & -1.1858  \\
    $M_{4}$ & 13.42   & 8.02    & 11.74   & 18.86   & 15.75   & 10.60   & 11.57   & 19.07    \\
    Med     & 0.9469  & 0.4485  & 0.8686  & 0.7920  & 0.6945  & 0.3143  & 0.8366  & 0.6382   \\
    \end{tabularx}
}



\RPprep{Income growth - Distributional tests}{1}{0}{FIGDdist}{%
    This table presents results of tests of distribution equality for the FIGD, based on the income measures described in Table~\ref{tab:DataDef}, as well as their time- and scale-adjusted versions (relative to total capital KT), denoted $\widetilde{XX}$. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a)-(c) report the test statistics and their p-values for the Stable, Laplace, and DLN, respectively. Panel (d) reports the relative likelihoods for each distribution. The raw variables (columns 1-4) use the \{Good\} data subset. The scale adjusted versions use the \{Non-Bank\} subset.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrr}
    \toprule
	& CF & CA & DI & DE & $\widetilde{\text{CF}}$ & $\widetilde{\text{CA}}$ & $\widetilde{\text{DI}}$ & $\widetilde{\text{DE}}$\\ 
	\midrule
    \\ \multicolumn{9}{l}{\textit{Panel (a): FIGD vs. Stable}}\\
	\midrule
    K-S   & 0.066 & 0.008 & 0.031 & 0.045  & 0.014 & 0.007 & 0.030 & 0.020  \\
    p-val & 0.008 & 0.070 & 0.024 & 0.015  & 0.046 & 0.079 & 0.024 & 0.036  \\
    C-2   & 486   & 59    & 342   & $>$999 & 120   & 42    & 344   & 183    \\
    p-val & 0.015 & 0.049 & 0.019 & 0.006  & 0.035 & 0.057 & 0.019 & 0.028  \\
    A-D   & 63.91 & 2.96  & 13.03 & 24.09  & 5.86  & 2.12  & 13.48 & 4.72   \\
    p-val & 0.012 & 0.051 & 0.030 & 0.022  & 0.041 & 0.057 & 0.029 & 0.044  \\
    \\ \multicolumn{9}{l}{\textit{Panel (a): FIGD vs. Laplace}}\\
	\midrule
    K-S   & 0.078  & 0.082  & 0.042 & 0.062  & 0.073  & 0.070  & 0.043 & 0.045  \\
    p-val & 0.004  & 0.004  & 0.017 & 0.009  & 0.006  & 0.006  & 0.016 & 0.015  \\
    C-2   & $>$999 & $>$999 & 555   & $>$999 & $>$999 & $>$999 & 570   & $>$999 \\
    p-val & 0.001  & 0.000  & 0.014 & 0.000  & 0.002  & 0.003  & 0.013 & 0.005  \\
    A-D   & 116.2  & 165.1  & 22.81 & 85.91  & 105.8  & 116.9  & 23.26 & 64.98  \\
    p-val & 0.006  & 0.003  & 0.023 & 0.009  & 0.007  & 0.006  & 0.023 & 0.012  \\
    \\ \multicolumn{9}{l}{\textit{Panel (c): FIGD vs. DLN}}\\
	\midrule
    K-S   & 0.009 & 0.005 & 0.024 & 0.033 & 0.007 & 0.005 & 0.026 & 0.015  \\
    p-val & 0.065 & 0.094 & 0.031 & 0.022 & 0.074 & 0.095 & 0.028 & 0.044  \\
    C-2   & 88    & 18    & 327   & 648   & 59    & 25    & 366   & 218    \\
    p-val & 0.040 & 0.085 & 0.020 & 0.012 & 0.049 & 0.073 & 0.019 & 0.026  \\
    A-D   & 1.85  & 0.54  & 10.63 & 12.12 & 1.11  & 0.69  & 12.03 & 3.78   \\
    p-val & 0.059 & 0.086 & 0.032 & 0.031 & 0.070 & 0.080 & 0.031 & 0.047  \\
    \\ \multicolumn{9}{l}{\textit{Panel (d): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
}



\RPprep{Investment - Descriptive statistics}{0}{0}{FNDDescMom}{%
    The first four columns of this table present statistics for the positive side of the FND (incl. depreciation DP), while the next three concentrate on the negative side and the last four on the entire investment intensity distribution (i.e., investment divided by total capital KT, and DP/KP). Variable definitions are in Table~\ref{tab:DataDef}. The positive and negative sides are in asinh scale. $M_1$ to $M_4$ are the first four central moments. Persistence for the positives and negatives is the 1-lag pooled auto-correlation, while for intensities it is the \cite{ArellanoBover1995}/\cite{BlundellBond1998} panel estimate. \%Ob is the percent of total observations in the positive/negative side, and may not sum to 100\% due to zero-valued obs. The scaling coefficient is the slope in a quantile regression of (asinh) income or of intensity on scale. All values are based on the \{Non-Bank\} data subset.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrrr}
    \toprule
	& IT$^{+}$ & IP$^{+}$ & IA$^{+}$ & DP & IT$^{-}$ & IP$^{-}$ & IA$^{-}$ & $\widetilde{\text{IT}}$ & $\widetilde{\text{IP}}$ & $\widetilde{\text{IA}}$ & $\widetilde{\text{DP}}$\\
	\midrule
    $M_{1}$       & 4.99 & 4.04 & 4.02 & 3.16 & -4.28 & -3.15 & -2.45 & 0.09 & 0.07 & 0.08 & 0.26  \\
    $M_{2}$       & 2.10 & 2.19 & 2.24 & 2.11 & 2.05  & 2.25  & 1.78  & 0.36 & 0.16 & 0.12 & 0.32  \\
    $M_{3}$       & 0.15 & 0.33 & 0.34 & 0.37 & -0.35 & -0.57 & -0.61 & 3.96 & 6.99 & 7.39 & 7.74  \\
    $M_{4}$       & 2.89 & 2.68 & 2.63 & 2.89 & 2.96  & 2.67  & 2.84  & 35   & 126  & 136  & 123   \\
    Pers.         & 0.24 & 0.51 & 0.87 & 0.99 & 0.08  & -0.06 & -0.23 & 0.10 & 0.14 & 0.26 & 0.07  \\
    \%Ob          & 0.63 & 0.85 & 0.96 & /    & 0.37  & 0.15  & 0.03  & /    & /    & /    & /     \\
    $\beta_{scl}$ & 0.89 & 0.98 & 1.03 & 0.86 & -0.86 & -0.94 & -0.77 & 0.00 & 0.00 & 0.00 & -0.02 \\
    \end{tabularx}
}



\RPprep{Investment - Distributional tests}{1}{0}{FNDdist}{%
    This table presents results of tests of distribution equality for the FND, based on the investment measures described in Table~\ref{tab:DataDef}, as well as their intensities relative to total capital KT, denoted $\widetilde{XX}$. K-S is a Kolmogorov–Smirnov test; C-2 is a binned $\chi^2$ test with 50 bins; A-D is an Anderson-Darling test. Panels (a)-(c) report the test statistics and their p-values for the Stable, Laplace, and DLN, respectively. Panel (d) reports the relative likelihoods for each distribution. All values are based on the \{Non-Bank\} data subset.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrr}
    \toprule
	& IT & IP & IA & $\widetilde{\text{IT}}$ & $\widetilde{\text{IP}}$ & $\widetilde{\text{IA}}$ \\ 
	\midrule
    \\ \multicolumn{7}{l}{\textit{Panel (a): FND vs. Stable}}\\
	\midrule
    K-S   & 0.026 & 0.048 & 0.067  & 0.020 & 0.120 & 0.068  \\
    p-val & 0.028 & 0.014 & 0.007  & 0.036 & 0.000 & 0.007  \\
    C-2   & 380   & 728   & $>$999 & 193 & $>$999  & $>$999 \\
    p-val & 0.018 & 0.011 & 0.005  & 0.027 & 0.002 & 0.007  \\
    A-D   & 13.75 & 56.04 & 112.0  & 12.25 & 188.1 & 76.00  \\
    p-val & 0.029 & 0.013 & 0.007  & 0.031 & 0.002 & 0.010  \\
    \\ \multicolumn{7}{l}{\textit{Panel (a): FND vs. Laplace}}\\
	\midrule
    K-S   & 0.279  & 0.350  & 0.444  & 0.079 & 0.081  & 0.064  \\
    p-val & 0.000  & 0.000  & 0.000  & 0.004 & 0.004  & 0.008  \\
    C-2   & $>$999 & $>$999 & $>$999 & 924   & $>$999 & $>$999 \\
    p-val & 0.000  & 0.000  & 0.000  & 0.008 & 0.002  & 0.007  \\
    A-D   & $>$999 & $>$999 & $>$999 & 93.14 & 145.9  & 95.42  \\
    p-val & 0.000  & 0.000  & 0.000  & 0.008 & 0.004  & 0.008  \\
    \\ \multicolumn{7}{l}{\textit{Panel (c): FND vs. DLN}}\\
	\midrule
    K-S   & 0.006 & 0.004 & 0.007 & 0.008 & 0.006 & 0.013  \\
    p-val & 0.086 & 0.127 & 0.074 & 0.071 & 0.082 & 0.049  \\
    C-2   & 27    & 14    & 45    & 42    & 29    & 82     \\
    p-val & 0.070 & 0.099 & 0.055 & 0.057 & 0.068 & 0.042  \\
    A-D   & 0.84  & 0.18  & 1.41  & 1.84  & 1.25  & 3.72   \\
    p-val & 0.076 & 0.121 & 0.065 & 0.059 & 0.067 & 0.047  \\
    \\ \multicolumn{7}{l}{\textit{Panel (d): Distribution comparison}}\\
	\midrule
	\multicolumn{2}{l}{AIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\multicolumn{2}{l}{BIC R.L.:} \\
    Stable  & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    Laplace & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
    DLN     & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
	\bottomrule
    \end{tabularx}
}



\RPprep{R\&D - Descriptive statistics}{0}{0}{FRDDescMom}{%
    This table presents moments of (log) R\&D and physical investment intensities. The first two columns describe R\&D intensities relative to KT and SL. The next four describe physical intensities for R\&D-performing firms, and the last four repeat for non-R\&D-performing firms. Only positive investments are considered. Panel (a) describes the first four moments of each distribution, its persistence of investment based on the \cite{ArellanoBover1995}/\cite{BlundellBond1998} panel estimator, and its coefficient of decreasing median with scale. Panels (b)-(d) reports results of skewness-median regressions, for all firms, small firms ($<\$100$M in KT or SL), and large firms ($>\$100$M), respectively.
}
\RPtab{%
    \begin{tabularx}{\linewidth}{Frrrrrrrrrr}
    \toprule
    & & & \multicolumn{4}{c}{R\&D-performing} & \multicolumn{4}{c}{non-R\&D-performing} \\
	log of & $\frac{RD}{KT}$ & $\frac{RD}{SL}$ & $\frac{IP}{KT}$ & $\frac{IP}{SL}$ & $\frac{IA}{KT}$ & $\frac{IA}{SL}$ & $\frac{IP}{KT}$ & $\frac{IP}{SL}$ & $\frac{IA}{KT}$ & $\frac{IA}{SL}$\\
	\midrule
    \\ \multicolumn{11}{l}{\textit{Panel (a): Descriptive moments}}\\
	\midrule
    $M_{1}$       & -3.171 & -3.022 & -3.301 & -3.120 & -3.399 & -3.224 & -3.074 & -3.154 & -3.143 & -3.184 \\
    $M_{2}$       & 1.413  & 1.730  & 1.106 & 1.237 & 1.063 & 1.136 & 1.280 & 1.580 & 1.201 & 1.501  		\\
    $M_{3}$       & -0.709 & 0.092  & -0.957 & -0.207 & -0.737 & 0.133 & -0.631 & 0.033 & -0.681 & 0.115  	\\
    $M_{4}$       & 3.791  & 4.039  & 6.349 & 5.801 & 5.464 & 5.642 & 4.825 & 3.978 & 4.917 & 3.862  		\\
    Pers.         & 0.706  & 0.673  & 0.217 & 0.212 & 0.381 & 0.352 & 0.158 & 0.191 & 0.386 & 0.390  		\\
    $\beta_{scl}$ & -0.239 & -0.339 & 0.019 & -0.030 & 0.080 & 0.031 & -0.004 & -0.124 & 0.058 & -0.055  	\\
    \\ \multicolumn{11}{l}{\textit{Panel (b): Binned skewness-median regressions - All firms}}\\
	\midrule
    $\beta_{med}$ & -0.173 & -0.057 & 0.126 & 0.070 & 0.101 & 0.081 & -0.200 & 0.009 & -0.810 & -0.163  	\\
    s.e.          & 0.027 & 0.038 & 0.157 & 0.066 & 0.067 & 0.076 & 0.174 & 0.060 & 0.086 & 0.087  			\\
	sig			  & *** & ~ & ~ & ~ & ~ & ~ & ~ & ~ & *** &   												\\
    R$^2$     & 0.462 & 0.024 & -0.008 & 0.002 & 0.026 & 0.003 & 0.007 & -0.021 & 0.647 & 0.050  		\\
    \\ \multicolumn{11}{l}{\textit{Panel (c): Binned skewness-median regressions - small firms}}\\
	\midrule
    $\beta_{med}$ & -1.193 & 0.044 & 1.387 & 0.049 & -0.419 & -0.063 & -0.058 & -0.215 & -0.130 & -0.275  	\\
    s.e.          & 0.737 & 0.080 & 0.387 & 0.067 & 0.347 & 0.060 & 0.208 & 0.028 & 0.243 & 0.047  			\\
	sig			  & ~ & ~ & *** & ~ & ~ & ~ & ~ & *** & ~ & ***  											\\
    R$^2$     & 0.128 & -0.057 & 0.542 & -0.039 & 0.044 & 0.008 & -0.152 & 0.904 & -0.113 & 0.844  		\\
    \\ \multicolumn{11}{l}{\textit{Panel (d): Binned skewness-median regressions - large firms}}\\
	\midrule
    $\beta_{med}$ & -0.214 & -0.371 & 0.019 & -0.797 & 0.285 & 0.638 & -0.286 & 0.291 & -1.066 & -0.567  	\\
    s.e.          & 0.030 & 0.027 & 0.221 & 0.280 & 0.091 & 0.147 & 0.223 & 0.158 & 0.113 & 0.249  			\\
	sig			  & *** & *** & ~ & ** & ** & *** & ~ & ~ & *** & *  										\\
    R$^2$     & 0.585 & 0.851 & -0.028 & 0.169 & 0.193 & 0.337 & 0.016 & 0.055 & 0.687 & 0.092  		\\
\end{tabularx}
}



